Taxonomy-guided Semantic Indexing for Academic Paper Search

Academic paper search is an essential task for efficient literature discovery and scientific advancement. While dense retrieval has advanced various ad-hoc searches, it often struggles to match the underlying academic concepts between queries and documents, which is critical for paper search. To enable effective academic concept matching for paper search, we propose Taxonomy-guided Semantic Indexing (TaxoIndex) framework. TaxoIndex extracts key concepts from papers and organizes them as a semantic index guided by an academic taxonomy, and then leverages this index as foundational knowledge to identify academic concepts and link queries and documents. As a plug-and-play framework, TaxoIndex can be flexibly employed to enhance existing dense retrievers. Extensive experiments show that TaxoIndex brings significant improvements, even with highly limited training data, and greatly enhances interpretability.

==> sections/991main_table_original.tex <==




\begin{table*}[t]
\centering
\resizebox{1.\linewidth}{!}{%
\begin{tabular}{c lcccccc|cccccc} \toprule
& & \multicolumn{6}{c|}{CSFCube} & \multicolumn{6}{c}{DORIS-MAE} \\ \cmidrule(lr){3-8}\cmidrule(lr){9-14}
& & N@5 & N@10 & N@20 & R@20 & R@50 & R@100 & N@5 & N@10 & N@20 & R@20 & R@50 & R@100 \\ \midrule
& BM25 & 0.3069 & 0.3098 & 0.3169 & 0.3275 & 0.5043 & 0.6354 &  0.3540 & 0.3296 & 0.3371 & 0.2921 & 0.4897 & 0.6691 \\ \midrule
\parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{SPECTER-v2}}} 
& no Fine-Tuning & 0.3515 & 0.3370 & 0.3381 & 0.3144 & 0.5244 & 0.6804  & 0.3846 & 0.3602 & 0.3661 & 0.3221 & 0.5505 & 0.7088 \\
& FFT & 0.3723 & 0.3682 & 0.3668 & 0.3610 & 0.5760 & 0.6918  & 0.4078 & 0.3870 & 0.3878 & 0.3419 & 0.5621 & 0.7359 \\
& aFT & 0.3775 & 0.3437 & 0.3668 & 0.3566 & 0.5778 & 0.6962  & 0.4002 & 0.3715 & 0.3855 & 0.3441 & 0.5581 & 0.7138 \\ \cmidrule(lr){2-14}
& FFT w/ GRF & 0.3307 & 0.3170 & 0.3392 & 0.3335 & 0.5605 & 0.7050  & 0.3999 & 0.3788 & 0.3884 & 0.3461 & \textbf{0.5857} & \underline{0.7555} \\
& FFT w/ ToTER & 0.4055 & 0.3747 & 0.3989 & 0.3750 & 0.5907 & 0.7104  & 0.4232 & 0.3944 & \underline{0.4002} & \underline{0.3499} & 0.5628 & 0.7362 \\ \cmidrule(lr){2-14}
& JTR & 0.3788 & 0.3520 & 0.3877 & \underline{0.4008} & 0.5977 & 0.6992  & 0.3953 & 0.3798 & 0.3851 & 0.3312 & 0.5484 & 0.7129 \\
& \cellcolor{gray!15}\proposed & \cellcolor{gray!15} \underline{0.4582}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.4170}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.4249}$^{\dagger *}$ & \cellcolor{gray!15} 0.3966$^{\dagger}$ & \cellcolor{gray!15} \textbf{0.6331}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.7414}$^{\dagger *}$  & \cellcolor{gray!15} \underline{0.4470}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.4208}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4216}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.3503} & \cellcolor{gray!15} 0.5775$^{\dagger}$ & \cellcolor{gray!15} \textbf{0.7561}$^{\dagger}$ \\
& \cellcolor{gray!15}\proposed++ & \cellcolor{gray!15} \textbf{0.4694}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4262}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4307}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4046}$^{\dagger}$ & \cellcolor{gray!15} \underline{0.6212}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.7457}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4486}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4240}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4216}$^{\dagger *}$ & \cellcolor{gray!15} 0.3494 & \cellcolor{gray!15} \underline{0.5805}$^{\dagger}$ & \cellcolor{gray!15} \textbf{0.7507}$^{\dagger}$ \\ \midrule
\parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Contriever-MS}}} 
& no Fine-Tuning & 0.3402 & 0.3108 & 0.3365 & 0.3333 & 0.5512 & 0.6816  & 0.4272 & 0.3981 & 0.3768 & 0.3013 & 0.5073 & 0.6352 \\
& FFT & 0.3636 & 0.3283 & 0.3653 & 0.3852 & 0.5894 & 0.7046  & 0.4532 & 0.4070 & 0.3960 & 0.3308 & 0.5103 & 0.6523 \\
& aFT & 0.3456 & 0.3277 & 0.3617 & 0.3850 & 0.5780 & 0.7109 & 0.4391 & 0.4017 & 0.3906 & 0.3291 & 0.5072 & 0.6483 \\ \cmidrule(lr){2-14}
& FFT w/ GRF & 0.3534 & 0.3126 & 0.3469 & 0.3571 & 0.5591 & 0.6687  & 0.4465 & 0.3808 & 0.3717 & 0.2988 & 0.5113 & 0.6431 \\
& FFT w/ ToTER & 0.3749 & 0.3534 & 0.3791 & 0.3860 & \textbf{0.5965} & \underline{0.7248}  & 0.4575 & \textbf{0.4230} & 0.4028 & 0.3312 & 0.5386 & 0.7025 \\ \cmidrule(lr){2-14}
& JTR & 0.3510 & 0.3310 & 0.3599 & 0.3753 & 0.5783 & 0.7136 & 0.4352 & 0.4078 & 0.3951 & 0.3283 & 0.5161 & 0.6668 \\
& \cellcolor{gray!15}\proposed & \cellcolor{gray!15} \underline{0.4003}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.3859}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.4089}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.4170}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.5962}$^{\dagger}$ & \cellcolor{gray!15} \textbf{0.7258}$^{\dagger}$  & \cellcolor{gray!15} \underline{0.4610} & \cellcolor{gray!15} \underline{0.4228}$^{\dagger}$ & \cellcolor{gray!15} \underline{0.4123}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.3507}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.5567}$^{\dagger *}$ & \cellcolor{gray!15} \underline{0.7290}$^{\dagger *}$ \\
& \cellcolor{gray!15}\proposed++ & \cellcolor{gray!15} \textbf{0.4211}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.3861}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4107}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4171}$^{\dagger}$ & \cellcolor{gray!15} 0.5945 & \cellcolor{gray!15} \textbf{0.7258}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.4626} & \cellcolor{gray!15} 0.4224$^{\dagger}$ & \cellcolor{gray!15} \textbf{0.4139}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.3508}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.5602}$^{\dagger *}$ & \cellcolor{gray!15} \textbf{0.7325}$^{\dagger *}$ \\ \bottomrule
\end{tabular}}
\caption{Retrieval performance comparison on CSFCube and DORIS-MAE datasets. $^{\dagger}$ and * indicate the statistically significant difference (paired t-test, $p<0.05$) from FFT and the best baseline, respectively.}
\label{tab:main}
\vspace{-0.3cm}
\end{table*}



\begin{table}[t]
\centering
\resizebox{1.02\linewidth}{!}{%
\begin{tabular}{ccllllll} \toprule
\multirow{2}{*}{\parbox{0.7cm}{\centering Train\\ data}} & \multirow{2}{*}{} & \multicolumn{3}{c}{\csfcube} & \multicolumn{3}{c}{\dorismae} \\  \cmidrule(lr){3-5} \cmidrule(lr){6-8}
\multicolumn{1}{l}{\textbf{}} &  & N@5 & N@10 & R@50 & N@5 & N@10 & R@50 \\ \midrule
% \multicolumn{2}{c}{no Fine-Tuning}  & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ \midrule
\multirow{2}{*}{100\%} & FFT & +5.92\% & +9.26\% & +9.84\% & +6.09\% & +2.24\% & +0.59\% \\
 & TSI$^\dagger$ & +\textbf{30.36}\% & +\textbf{23.74}\% & +\textbf{20.73}\% & +\textbf{7.91}\% & +\textbf{6.20}\% & +\textbf{9.74}\% \\ \midrule
\multirow{2}{*}{50\%} & FFT & +0.80\% & +4.57\% & +7.91\% & +3.46\% & +1.98\% & \cellcolor{red!15} - 0.12\% \\
 & TSI$^\dagger$ & +\textbf{20.65}\% & +\textbf{18.40}\% & +\textbf{19.26}\% & +\textbf{7.58}\% & +\textbf{6.13}\% & +\textbf{8.40}\% \\ \midrule
\multirow{2}{*}{10\%} & FFT & +0.51\% & +1.36\% & +0.40\% & +2.29\% & +0.30\% & \cellcolor{red!15} - 0.41\% \\
 & TSI$^\dagger$ & +\textbf{19.63}\% & +\textbf{14.36}\% & +\textbf{15.64}\% & +\textbf{6.76}\% & +\textbf{5.85}\% & +\textbf{7.69}\% \\ \bottomrule
\end{tabular}}
\caption{Results of FFT and \proposed with varying amounts of training data. 
We report improvements over no Fine-Tuning. 
$^\dagger$ denotes $p < 0.05$ from paired t-test with FFT. }
\label{tab:limited_data}
\end{table}


\begin{table}[t]
\centering
% \renewcommand{\arraystretch}{0.85}
%\renewcommand{\tabcolsep}{1.3mm}
\resizebox{1.02\linewidth}{!}{%
\begin{tabular}{clllllll} \toprule
&  & \multicolumn{3}{c}{(a) High lexical mismatch} &  \multicolumn{3}{c}{(b) High topic diversity} \\  \cmidrule(lr){3-5} \cmidrule(lr){6-8}
&  & N@5    & N@10   & R@50   & N@5    & N@10   & R@50   \\ \midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\small CSFCube}} & FFT & +5.81\%& \cellcolor{red!15} - 0.39\%	& \cellcolor{red!15} - 1.45\%&	+5.01\%&	+6.25\%&	+0.78\% \\
& ToTER & +16.19\%&+11.86\%&+11.78\%&+5.10\%&	+10.64\%&+10.90\% \\
& TSI & +\textbf{56.35}\%$^*$&	+\textbf{47.48}\%$^*$&+\textbf{16.94}\%$^*$&+\textbf{50.22}\%$^*$&+\textbf{41.66}\%$^*$&+\textbf{11.25}\% \\ \midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\small DORIS-M}} & FFT   & +1.04\%&	+1.99\%&	+3.47\%&	+0.10\%&	+0.15\%&	\cellcolor{red!15}- 2.21\% \\
& ToTER &+1.07\%&	+3.28\%&	+14.24\%&	+6.90\%&	+3.79\%&	+4.78\% \\
& TSI   & +\textbf{8.58}\%$^*$&	+\textbf{7.09}\%$^*$&	+\textbf{24.65}\%$^*$&	+\textbf{10.41}\%$^*$& +\textbf{4.17}\%&	+\textbf{11.16}\%$^*$ \\ \bottomrule
\end{tabular}}
\caption{Further analysis for \textit{difficult queries}. We report improvement over no Fine-Tuning. $^*$ denotes $p < 0.05$ from paired t-test with ToTER.}
\label{tab:difficult}
\end{table}

==> sections/9990Intro_old.tex <==
\begin{figure*}[t]
\centering    \includegraphics[width=1.\linewidth]{sections/figure/intro_motivating_v6.pdf}
\caption{A motivating case study from \csfcube dataset. Results of (left) dense retrieval, (right) \proposed.
For the dense retriever, we use \specter fully fine-tuned on the target corpus. The detailed setup is provided~in~Appendix~\ref{A:case_study}.
}
\label{fig:motivating}
\end{figure*}



Academic paper search is essential for efficient literature discovery and facilitating access to technical solutions. 
Recently, dense retrieval has advanced in various ad-hoc searches \cite{karpukhin2020dense, CTR}.
It encodes queries and documents as dense embeddings, measuring relevance by embedding similarity.
These embeddings effectively capture textual semantics via pre-trained language models trained on massive corpora.
% Furthermore, recent studies for academic domain \cite{OAGBERT, SPECTER2} have successfully incorporated paper metadata (e.g., citations, affiliations) to further improve embedding quality. 



However, the existing methods often lack the capability of identifying specific academic concepts from the texts, which is critical for comprehending query intents and finding relevant papers.
We illustrate these challenges using a concrete example in Figure~\ref{fig:motivating}, which handles the query "\textit{learning to win by reading manuals in a Monte-Carlo framework}".

\textbf{First}, user queries often encompass various academic concepts in limited contexts, making it challenging to comprehend search intents.
Specifically, the query includes multiple concepts: optimizing decision-making for a task (learning to win) and acquiring knowledge from text (reading manuals).
It also implies a reinforcement learning solution using probabilistic sampling (Monte-Carlo).
Such detailed intents are usually not explicitly stated in queries.
Further, inferring them requires an inherent understanding of specialized contents, which is not sufficiently obtained from general corpora.


\textbf{Second}, relevance between queries and documents must be judged by jointly considering multiple academic concepts.
That is, an ideally relevant document should address all query concepts, rather than only partially covering them.
This requires identifying academic concepts commonly included in both queries and documents, and reflecting them for relevance prediction.
This is difficult due to discrepancies in expression (e.g., terminology choice, language style) between queries and documents, as well as the need for domain-specific~knowledge.

% A retriever should find documents covering all query concepts, rather than documents only partially covering them.



Figure \ref{fig:motivating}(left) shows dense retrieval results for the query, which ranks an irrelevant document (Paper A) at the top-1.
Although the paper includes `solving a goal' and `machine comprehension of text', which have similar semantics to `learning to win' and `reading manuals' in the query, it falls short of addressing the query concepts.
This shows that overall semantic similarity captured by dense retrievers can be insufficient to reflect specific academic concepts, leading to suboptimal~results.



To tackle these challenges, we propose a new approach that pre-organizes corpus knowledge by extracting key concepts from each paper. 
Prior to retrieval, we construct a \textit{semantic index} that stores semantic components best describing each paper. 
The proposed index represents each paper at two different granularities: topic and phrase levels, as shown in Figure \ref{fig:motivating}(right). 
Topic level provides a broader categorization of research, such as `reinforcement learning' or `natural language processing', while phrase level includes specific details, such as `text-based games' or `control policy', complementarily revealing each paper's concepts.
We utilize this index as a basis for identifying academic concepts and enhancing relevance~prediction.


We propose a Taxonomy-guided Semantic Indexing (\proposed) framework to improve dense retrieval-based paper search.
We first design a new index construction strategy that extracts core topics and phrases from each paper.
To guide this process, we propose using an academic taxonomy, a hierarchical tree structure outlining academic topics.\footnote{Academic taxonomies are widely used for study categorization in various institutions (e.g., \href{https://dl.acm.org/ccs}{ACM Computing Classification System}) and can be readily obtained from the web.}
We then introduce a new training strategy, called \textit{index learning}, that trains the model to explicitly identify the indexed information for input text.
This is a critical technique that enables \proposed to infer the most related academic concepts in test queries, even if expressed in different terms or not explicitly mentioned, by associating them with papers having similar contexts.
This inferred information helps identify relevant papers sharing academic concepts, combined with the semantic similarity from dense retrievers.
Figure \ref{fig:motivating}(right) shows that \proposed finds Paper B as the top-2 result based on high overlap in indexed information (highlighted~in~yellow).


\proposed provides several advantages over dense retrieval.
First, \proposed largely improves the retrieval quality by effectively capturing academic concepts.
Notably, index learning offers a new type of supervision to identify key concepts from each text, which is not directly provided by query-document training pairs, yielding significant improvements even with limited training data.
Second, \proposed enhances interpretability by explicitly representing each text with topics and phrases, as shown in our case studies.
Moreover, these advancements do not come at the large cost of model complexity. 
\proposed updates only a small module, accounting for 5.6\% of the model parameters, yet achieves significant improvements over~fully~fine-tuned~models.



Our contributions are summarized as follows:
(1) We propose \proposed, which systematically constructs and leverages semantic index, a new approach to improve dense retrieval.
(2) We design an index construction strategy that represents each paper at both topic and phrase levels, with the guidance of academic taxonomy.
(3) We introduce an index learning strategy that enables the model to identify the most related concepts from an input text.
(4) We validate the effectiveness of \proposed by extensive experiments. We also provide a comprehensive ablation and case studies of our~proposed~approach.




